On the Optimality of D2D Coded Caching with Uncoded Cache Placement and One-shot Delivery

We consider a cache-aided wireless device-to-device (D2D) network of the type introduced by Ji, Caire, and Molisch [1], where the placement phase is orchestrated by a central server. We assume that the devices' caches are filled with uncoded data, and the whole content database is contained in the collection of caches. After the cache placement phase, the files requested by the users are serviced by inter-device multicast communication. For such a system setting, we provide the exact characterization of the optimal load-memory trade-off under the assumptions of uncoded placement and one-shot delivery. In particular, we derive both the minimum average (under uniformly distributed demands) and the minimum worst-case sum-load of the D2D transmissions, for given individual cache memory size at disposal of each user. Furthermore, we show that the performance of the proposed scheme is within factor $4$ of the information-theoretic optimum. Capitalizing on the one-shot delivery property, we also propose an extension of the presented scheme that provides robustness against random user inactivity.

==> fig2a.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.522in,
at={(0.758in,0.525in)},
scale only axis,
xmin=1,
xmax=6,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={M},
ymin=0,
ymax=9,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Load},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
1	9\\
1.33333333333333	6.5\\
1.66666666666667	5\\
2	4\\
2.33333333333333	3.28571428571429\\
2.66666666666667	2.75\\
3	2.33333333333333\\
3.33333333333333	2\\
3.66666666666667	1.72727272727273\\
4	1.5\\
4.33333333333333	1.30769230769231\\
4.66666666666667	1.14285714285714\\
5	1\\
5.33333333333333	0.875\\
5.66666666666667	0.764705882352941\\
6	0.666666666666667\\
};
\addlegendentry{Scheme Ji et al. \cite{ji2016fundamental}}

\addplot [color=black, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	6.61330049261083\\
1.33333333333333	5.4392446633826\\
1.66666666666667	4.51042061386889\\
2	3.77152961980548\\
2.33333333333333	3.17963875205254\\
2.66666666666667	2.70157421289355\\
3	2.31181076128602\\
3.33333333333333	1.99077604055115\\
3.66666666666667	1.72349928931638\\
4	1.49854358535018\\
4.33333333333333	1.30716949217699\\
4.66666666666667	1.14268579995716\\
5	0.999950024987506\\
5.33333333333333	0.874987506246877\\
5.66666666666667	0.764703362604412\\
6	0.666666300549359\\
};
\addlegendentry{Proposed scheme}

\addplot [color=mycolor1, dashdotted, line width=2.0pt]
  table[row sep=crcr]{%
1	5.55665024630542\\
1.33333333333333	4.63426382047072\\
1.66666666666667	3.89467811881605\\
2	3.29801692560313\\
2.33333333333333	2.81312260536398\\
2.66666666666667	2.4157476817147\\
3	2.08708645677161\\
3.33333333333333	1.81259153972797\\
3.66666666666667	1.58102734347112\\
4	1.38371912944627\\
4.33333333333333	1.21396206658575\\
4.66666666666667	1.06656005330668\\
5	0.937468765617191\\
5.33333333333333	0.82352157254706\\
5.66666666666667	0.722220635713889\\
6	0.631578716136437\\
};
\addlegendentry{Shared-link scheme \cite{yu2018exact}}

\addplot [color=green, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	3.23076923076923\\
1.33333333333333	2.46153846153846\\
1.66666666666667	1.88888888888889\\
2	1.42857142857143\\
2.33333333333333	1.25\\
2.66666666666667	1.07142857142857\\
3	0.931034482758621\\
3.33333333333333	0.862068965517241\\
3.66666666666667	0.793103448275862\\
4	0.724137931034483\\
4.33333333333333	0.655172413793104\\
4.66666666666667	0.586206896551724\\
5	0.517241379310345\\
5.33333333333333	0.482758620689655\\
5.66666666666667	0.448275862068966\\
6	0.413793103448276\\
};
\addlegendentry{Converse Sengupta et al. \cite{sengupta2015beyond}}

\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
1	2.5\\
1.33333333333333	1.66666666666667\\
1.66666666666667	1.33333333333333\\
2	1.2\\
2.33333333333333	1.06666666666667\\
2.66666666666667	0.933333333333333\\
3	0.8\\
3.33333333333333	0.689655172413793\\
3.66666666666667	0.655172413793103\\
4	0.620689655172414\\
4.33333333333333	0.586206896551724\\
4.66666666666667	0.551724137931034\\
5	0.517241379310345\\
5.33333333333333	0.482758620689655\\
5.66666666666667	0.448275862068966\\
6	0.413793103448276\\
};
\addlegendentry{Converse Ji et al. \cite{ji2016fundamental}}

\end{axis}
\end{tikzpicture}%

==> fig2b.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.522in,
at={(0.758in,0.525in)},
scale only axis,
xmin=1,
xmax=6,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={M},
ymin=0,
ymax=9,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Load},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={at={(0.516,0.757)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
1	8.94833333333333\\
1.33333333333333	6.5\\
1.66666666666667	5\\
2	4\\
2.33333333333333	3.28571428571434\\
2.66666666666667	2.75\\
3	2.33333333333324\\
3.33333333333333	2\\
3.66666666666667	1.7272727272727\\
4	1.5\\
4.33333333333333	1.30769230769236\\
4.66666666666667	1.14285714285721\\
5	1\\
5.33333333333333	0.875\\
5.66666666666667	0.764705882352953\\
6	0.666666666666696\\
};
\addlegendentry{Scheme Ji et al. \cite{ji2016fundamental}}

\addplot [color=black, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	6.42173133552269\\
1.33333333333333	5.31030857203674\\
1.66666666666667	4.43279480676838\\
2	3.72209820779477\\
2.33333333333333	3.15102199830181\\
2.66666666666667	2.68461619207494\\
3	2.30275774538533\\
3.33333333333333	1.9860251287898\\
3.66666666666667	1.72106506778357\\
4	1.49732548868421\\
4.33333333333333	1.30655984599479\\
4.66666666666667	1.14243821930303\\
5	0.999847224720976\\
5.33333333333333	0.874951130545828\\
5.66666666666667	0.764692374765\\
6	0.666663124335249\\
};
\addlegendentry{Proposed scheme}

\addplot [color=mycolor1, dashdotted, line width=2.0pt]
  table[row sep=crcr]{%
1	5.42853932676539\\
1.33333333333333	4.55870984613531\\
1.66666666666667	3.84613029626796\\
2	3.26944888046825\\
2.33333333333333	2.79666305973081\\
2.66666666666667	2.4057619808897\\
3	2.08174532197782\\
3.33333333333333	1.80962515163777\\
3.66666666666667	1.5795452581646\\
4	1.38297949735749\\
4.33333333333333	1.21362656079371\\
4.66666666666667	1.06642585373974\\
5	0.937407263035159\\
5.33333333333333	0.823500814037418\\
5.66666666666667	0.722213902731163\\
6	0.631576517601961\\
};
\addlegendentry{Shared-link scheme \cite{yu2018exact}}

\end{axis}
\end{tikzpicture}%

==> fig3a.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,1.00000,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.522in,
at={(0.758in,0.525in)},
scale only axis,
xmin=1.97355008600735,
xmax=14.9549257788443,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={M},
ymin=-0.217256415269162,
ymax=57.3478737600829,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Load},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=cyan, line width=2.0pt]
table[row sep=crcr]{%
	1.46363098758136	71.7179183914867\\
	2.18510888758092	47.1012360211887\\
	2.89982425307554	34.7978910369064\\
	3.60787172011657	27.4198250728859\\
	4.3093441671504	22.5043528728965\\
	5.00433275563232	18.9960386234206\\
	5.69292696952265	16.3671650373776\\
	6.37521465369205	14.3245563823698\\
	7.05128205128178	12.6923076923072\\
	7.72121384004555	11.3584798638687\\
	8.38509316770202	10.2484472049691\\
	9.04300168634053	9.31054611493049\\
	9.69501958589833	8.5078743304822\\
	10.3412256267406	7.81337047353738\\
	10.9816971713811	7.20673876871882\\
	11.6165102153506	6.67245915483804\\
	12.245739417262	6.19846069268816\\
	12.8694581280784	5.77521389681079\\
	13.4877384196186	5.39509536784744\\
	14.100651112317	5.0519339586079\\
	14.708265802269	4.74068071312801\\
	15.3106508875737	4.45716490866985\\
	15.9078735940017	4.197911087306\\
	16.4999999999999	3.95999999999998\\
	17.0870950610732	3.74096164058999\\
	17.6692226335269	3.53869205006164\\
	18.2464454976305	3.35138794854437\\
	18.8188253801785	3.17749489177806\\
	19.3864229765014	3.01566579634466\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 3.2 }\times\text{ 10}^{\text{-10}}\text{, a = 32}$}

\addplot [color=blue, dashed, line width=2.0pt]
table[row sep=crcr]{%
	1.46363098758136	54.3317563571868\\
	2.18510888758092	41.5685697469096\\
	2.89982425307554	32.8393093327048\\
	3.60787172011657	26.688783024255\\
	4.3093441671504	22.2235063639022\\
	5.00433275563232	18.8864284028326\\
	5.69292696952265	16.3240505792164\\
	6.37521465369205	14.3075554352531\\
	7.05128205128178	12.6856127011293\\
	7.72121384004555	11.355854410978\\
	8.38509316770202	10.2474242818124\\
	9.04300168634053	9.31015089160421\\
	9.69501958589833	8.50772315111286\\
	10.3412256267406	7.8133133047476\\
	10.9816971713811	7.20671742554543\\
	11.6165102153506	6.67245129810523\\
	12.245739417262	6.19845784445173\\
	12.8694581280784	5.77521288117748\\
	13.4877384196186	5.39509501205292\\
	14.100651112317	5.05193383630727\\
	14.708265802269	4.74068067193011\\
	15.3106508875737	4.45716489508778\\
	15.9078735940017	4.19791108292977\\
	16.4999999999999	3.95999999862391\\
	17.0870950610732	3.74096164016838\\
	17.6692226335269	3.53869204993598\\
	18.2464454976305	3.35138794850801\\
	18.8188253801785	3.17749489176786\\
	19.3864229765014	3.0156657963419\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 3.2 }\times\text{ 10}^{\text{-10}}\text{, a = 32}$}

\addplot [color=red, line width=2.0pt]
table[row sep=crcr]{%
	1.31160572337047	64.2686804451532\\
	1.96117274167986	42.2741679873215\\
	2.60663507109002	31.2796208530802\\
	3.24803149606295	24.6850393700784\\
	3.88540031397182	20.2904238618528\\
	4.51877934272277	17.1529175050293\\
	5.14820592823707	14.8010920436816\\
	5.7737169517885	12.9730430274754\\
	6.39534883720906	11.5116279069763\\
	7.01313755795998	10.3168469860899\\
	7.62711864406794	9.32203389830526\\
	8.23732718894	8.48103509393823\\
	8.84379785604916	7.76088383285947\\
	9.4465648854959	7.13740458015246\\
	10.0456621004566	6.59246575342468\\
	10.6411229135052	6.1122020887262\\
	11.2329803328288	5.68582955118496\\
	11.8212669683254	5.30483448440086\\
	12.4060150375941	4.96240601503762\\
	12.9872563718142	4.65303062754341\\
	13.5650224215246	4.37219730941702\\
	14.1393442622949	4.11617961511041\\
	14.7102526002977	3.88187221396746\\
	15.2777777777777	3.66666666666666\\
	15.8419497784347	3.46835586865138\\
	16.4027982326949	3.28505972835865\\
	16.9603524229076	3.11516677155446\\
	17.5146412884336	2.95728782753575\\
	18.065693430657	2.8102189781022\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 1. 3 }\times\text{ 10}^{\text{-5}}\text{, a = 24}$}

\addplot [color=green, dashed, line width=2.0pt]
table[row sep=crcr]{%
	1.31160572337047	48.6883942766311\\
	1.96117274167986	37.3085050184889\\
	2.60663507109002	29.5190632074392\\
	3.24803149606295	24.0269096517571\\
	3.88540031397182	20.0372064181075\\
	4.51877934272277	17.0539423919162\\
	5.14820592823707	14.7621029418915\\
	5.7737169517885	12.9576461095838\\
	6.39534883720906	11.5055557056754\\
	7.01313755795998	10.3144623011614\\
	7.62711864406794	9.32110344277851\\
	8.23732718894	8.48067508252119\\
	8.84379785604916	7.76074592702332\\
	9.4465648854959	7.13735235726307\\
	10.0456621004566	6.59244622945632\\
	10.6411229135052	6.11219489168871\\
	11.2329803328288	5.68582693850615\\
	11.8212669683254	5.30483355148882\\
	12.4060150375941	4.962405687778\\
	12.9872563718142	4.6530305148997\\
	13.5650224215246	4.37219727142134\\
	14.1393442622949	4.1161796025674\\
	14.7102526002977	3.88187220992069\\
	15.2777777777777	3.66666666539251\\
	15.8419497784347	3.46835586826049\\
	16.4027982326949	3.285059728242\\
	16.9603524229076	3.11516677152066\\
	17.5146412884336	2.95728782752626\\
	18.065693430657	2.81021897809963\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 1. 3 }\times\text{ 10}^{\text{-5}}\text{, a = 24}$}






\addplot [color=black, line width=2.0pt]
  table[row sep=crcr]{%
1.00000000000003	49.0000000000016\\
1.49999999999999	32.3333333333332\\
1.99999999999998	23.9999999999997\\
2.49999999999996	18.9999999999997\\
3.00000000000006	15.666666666667\\
3.49999999999981	13.2857142857136\\
3.99999999999995	11.4999999999999\\
4.50000000000001	10.1111111111111\\
4.99999999999982	8.99999999999967\\
5.50000000000013	8.09090909090928\\
6.00000000000012	7.33333333333348\\
6.49999999999994	6.69230769230763\\
7.00000000000013	6.14285714285726\\
7.49999999999977	5.66666666666649\\
8.00000000000003	5.25000000000002\\
8.49999999999996	4.88235294117645\\
8.99999999999981	4.55555555555546\\
9.49999999999968	4.2631578947367\\
10.0000000000001	4.00000000000003\\
10.5000000000001	3.76190476190479\\
11	3.54545454545454\\
11.4999999999998	3.34782608695647\\
12.0000000000005	3.16666666666679\\
12.5	3\\
13.0000000000003	2.84615384615392\\
13.4999999999999	2.70370370370368\\
14.0000000000001	2.5714285714286\\
14.5000000000002	2.448275862069\\
15.0000000000001	2.33333333333335\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 1, a = 0}$}

\addplot [color=mycolor1, dashed, line width=2.0pt]
table[row sep=crcr]{%
	1.00000000000003	37.1212121212133\\
	1.49999999999999	28.5353535353533\\
	1.99999999999998	22.6491721337079\\
	2.49999999999996	18.4934395501403\\
	3.00000000000006	15.4711521070721\\
	3.49999999999981	13.2090535617387\\
	3.99999999999995	11.4697066493969\\
	4.50000000000001	10.0991108466211\\
	4.99999999999982	8.99525264261898\\
	5.50000000000013	8.08903891981992\\
	6.00000000000012	7.33260137498577\\
	6.49999999999994	6.69202361057128\\
	7.00000000000013	6.14274798829847\\
	7.49999999999977	5.66662520485734\\
	8.00000000000003	5.24998445182159\\
	8.49999999999996	4.88234719227013\\
	8.99999999999981	4.55555346224553\\
	9.49999999999968	4.26315714501466\\
	10.0000000000001	3.99999973620894\\
	10.5000000000001	3.76190467083406\\
	11	3.5454545146435\\
	11.4999999999998	3.34782607675482\\
	12.0000000000005	3.16666666336561\\
	12.5	2.99999999895752\\
	13.0000000000003	2.84615384583316\\
	13.4999999999999	2.70370370360767\\
	14.0000000000001	2.5714285714007\\
	14.5000000000002	2.44827586206114\\
	15.0000000000001	2.33333333333121\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 1, a = 0}$}


\end{axis}
\end{tikzpicture}%

==> fig3b.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,1.00000,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.522in,
at={(0.758in,0.525in)},
scale only axis,
xmin=1.94493406103336,
xmax=14.8942428167937,
xlabel style={font=\bfseries\color{white!15!black}},
xlabel={M},
ymin=-0.100207610378118,
ymax=60.8351169567665,
ylabel style={font=\bfseries\color{white!15!black}},
ylabel={Load},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=cyan, line width=2.0pt]
table[row sep=crcr]{%
	1.46363098758136	63.4496717918412\\
	2.18510888758092	47.1012360212085\\
	2.89982425307554	34.7978910369064\\
	3.60787172011657	27.4198250728859\\
	4.3093441671504	22.5043528729057\\
	5.00433275563232	18.9960386234302\\
	5.69292696952265	16.3671650373776\\
	6.37521465369205	14.3245563823793\\
	7.05128205128178	12.6923076923072\\
	7.72121384004555	11.3584798638718\\
	8.38509316770202	10.248447204973\\
	9.04300168634053	9.31054611493419\\
	9.69501958589833	8.50787433048583\\
	10.3412256267406	7.81337047353638\\
	10.9816971713811	7.20673876871882\\
	11.6165102153506	6.67245915483598\\
	12.245739417262	6.19846069269229\\
	12.8694581280784	5.77521389680939\\
	13.4877384196186	5.39509536784744\\
	14.100651112317	5.05193395861114\\
	14.708265802269	4.74068071312948\\
	15.3106508875737	4.45716490867256\\
	15.9078735940017	4.19791108730711\\
	16.4999999999999	3.95999999999998\\
	17.0870950610732	3.74096164059152\\
	17.6692226335269	3.53869205006141\\
	18.2464454976305	3.35138794854483\\
	18.8188253801785	3.17749489178052\\
	19.3864229765014	3.01566579634544\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 3.2 }\times\text{ 10}^{\text{-10}}\text{, a = 32}$}

\addplot [color=blue, dashed, line width=2.0pt]
table[row sep=crcr]{%
	1.46363098758136	49.1150103636857\\
	2.18510888758092	38.8496334915879\\
	2.89982425307554	31.425059982889\\
	3.60787172011657	25.9696059551026\\
	4.3093441671504	21.8542048776329\\
	5.00433275563232	18.6999361323242\\
	5.69292696952265	16.2302559947271\\
	6.37521465369205	14.2609108400198\\
	7.05128205128178	12.6624551010769\\
	7.72121384004555	11.3445946108466\\
	8.38509316770202	10.2419242322634\\
	9.04300168634053	9.30749029532806\\
	9.69501958589833	8.50644868649798\\
	10.3412256267406	7.81271296426228\\
	10.9816971713811	7.20643721197461\\
	11.6165102153506	6.67232018187293\\
	12.245739417262	6.19839677342921\\
	12.8694581280784	5.77518498497825\\
	13.4877384196186	5.3950824164691\\
	14.100651112317	5.05192825038613\\
	14.708265802269	4.74067814352274\\
	15.3106508875737	4.45716379064739\\
	15.9078735940017	4.19791060511915\\
	16.4999999999999	3.9599997958292\\
	17.0870950610732	3.74096155232262\\
	17.6692226335269	3.53869201383501\\
	18.2464454976305	3.35138793342042\\
	18.8188253801785	3.1774948854584\\
	19.3864229765014	3.01566579390624\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 3.2 }\times\text{ 10}^{\text{-10}}\text{, a = 32}$}

\addplot [color=red, line width=2.0pt]
table[row sep=crcr]{%
	1.31160572337047	56.8592448330702\\
	1.96117274167986	42.2741679873393\\
	2.60663507109002	31.2796208530802\\
	3.24803149606295	24.6850393700784\\
	3.88540031397182	20.2904238618611\\
	4.51877934272277	17.1529175050379\\
	5.14820592823707	14.8010920436816\\
	5.7737169517885	12.973043027484\\
	6.39534883720906	11.5116279069763\\
	7.01313755795998	10.3168469860927\\
	7.62711864406794	9.32203389830878\\
	8.23732718894	8.4810350939416\\
	8.84379785604916	7.76088383286277\\
	9.4465648854959	7.13740458015155\\
	10.0456621004566	6.59246575342468\\
	10.6411229135052	6.11220208872431\\
	11.2329803328288	5.68582955118874\\
	11.8212669683254	5.30483448439958\\
	12.4060150375941	4.96240601503762\\
	12.9872563718142	4.65303062754639\\
	13.5650224215246	4.37219730941837\\
	14.1393442622949	4.11617961511291\\
	14.7102526002977	3.88187221396849\\
	15.2777777777777	3.66666666666666\\
	15.8419497784347	3.4683558686528\\
	16.4027982326949	3.28505972835844\\
	16.9603524229076	3.11516677155489\\
	17.5146412884336	2.95728782753804\\
	18.065693430657	2.81021897810293\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 1. 3 }\times\text{ 10}^{\text{-5}}\text{, a = 24}$}

\addplot [color=green, dashed, line width=2.0pt]
table[row sep=crcr]{%
	1.31160572337047	44.0135042527782\\
	1.96117274167986	34.8682130492382\\
	2.60663507109002	28.2478027334342\\
	3.24803149606295	23.3794615291344\\
	3.88540031397182	19.7042360042708\\
	4.51877934272277	16.8855448331003\\
	5.14820592823707	14.6772829822311\\
	5.7737169517885	12.915402404103\\
	6.39534883720906	11.4845523009767\\
	7.01313755795998	10.3042350844526\\
	7.62711864406794	9.31610057284978\\
	8.23732718894	8.47825152861681\\
	8.84379785604916	7.75958336027152\\
	9.4465648854959	7.13680395463145\\
	10.0456621004566	6.59218990014725\\
	10.6411229135052	6.11207478471011\\
	11.2329803328288	5.6857709182389\\
	11.8212669683254	5.30480792737821\\
	12.4060150375941	4.96239410236632\\
	12.9872563718142	4.6530253700458\\
	13.5650224215246	4.3721949395419\\
	14.1393442622949	4.11617858261972\\
	14.7102526002977	3.88187176808195\\
	15.2777777777777	3.66666647761963\\
	15.8419497784347	3.4683557868161\\
	16.4027982326949	3.28505969472853\\
	16.9603524229076	3.11516675749651\\
	17.5146412884336	2.95728782165407\\
	18.065693430657	2.81021897582991\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 1. 3 }\times\text{ 10}^{\text{-5}}\text{, a = 24}$}

\addplot [color=black, line width=2.0pt]
table[row sep=crcr]{%
	1.00000000000003	43.3508666666681\\
	1.49999999999999	32.3333333333468\\
	1.99999999999998	23.9999999999997\\
	2.49999999999996	18.9999999999997\\
	3.00000000000006	15.6666666666734\\
	3.49999999999981	13.2857142857203\\
	3.99999999999995	11.4999999999999\\
	4.50000000000001	10.1111111111179\\
	4.99999999999982	8.99999999999967\\
	5.50000000000013	8.09090909091153\\
	6.00000000000012	7.33333333333625\\
	6.49999999999994	6.69230769231029\\
	7.00000000000013	6.14285714285988\\
	7.49999999999977	5.66666666666577\\
	8.00000000000003	5.25000000000002\\
	8.49999999999996	4.88235294117494\\
	8.99999999999981	4.55555555555849\\
	9.49999999999968	4.26315789473567\\
	10.0000000000001	4.00000000000003\\
	10.5000000000001	3.76190476190721\\
	11	3.54545454545564\\
	11.4999999999998	3.3478260869585\\
	12.0000000000005	3.16666666666763\\
	12.5	3\\
	13.0000000000003	2.84615384615509\\
	13.4999999999999	2.70370370370351\\
	14.0000000000001	2.57142857142894\\
	14.5000000000002	2.44827586207089\\
	15.0000000000001	2.33333333333395\\
};
\addlegendentry{$\text{Scheme Ji et al. \cite{ji2016fundamental}, P}_{\text{out}}\text{ }\approx\text{ 1, a = 0}$}

\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1.00000000000003	33.5569626363606\\
1.49999999999999	26.668899920084\\
1.99999999999998	21.673768642744\\
2.49999999999996	17.9951006921216\\
3.00000000000006	15.21405858754\\
3.49999999999981	13.0786219980013\\
3.99999999999995	11.4038041110426\\
4.50000000000001	10.0661863585918\\
4.99999999999982	8.97883179894546\\
5.50000000000013	8.08101830259495\\
6.00000000000012	7.32866578397517\\
6.49999999999994	6.69011120621764\\
7.00000000000013	6.14182779909976\\
7.49999999999977	5.66618980640435\\
8.00000000000003	5.24978032048091\\
8.49999999999996	4.88225125227147\\
8.99999999999981	4.55550857812838\\
9.49999999999968	4.26313655254759\\
10.0000000000001	3.99999039766498\\
10.5000000000001	3.76190051129764\\
11	3.54545262370126\\
11.4999999999998	3.34782524719738\\
12.0000000000005	3.1666663029323\\
12.5	2.99999984532517\\
13.0000000000003	2.8461537789994\\
13.4999999999999	2.70370367602507\\
14.0000000000001	2.5714285598244\\
14.5000000000002	2.44827585719967\\
15.0000000000001	2.33333333144665\\
};
\addlegendentry{$\text{Proposed scheme, P}_{\text{out}}\text{ }\approx\text{ 1, a = 0}$}







\end{axis}
\end{tikzpicture}%
